Domain-General Crowd Counting in Unseen Scenarios

Domain shift across crowd data severely hinders crowd counting models to generalize to unseen scenarios. Although domain adaptive crowd counting approaches close this gap to a certain extent, they are still dependent on the target domain data to adapt (e.g. finetune) their models to the specific domain. In this paper, we aim to train a model based on a single source domain which can generalize well on any unseen domain. This falls into the realm of domain generalization that remains unexplored in crowd counting. We first introduce a dynamic sub-domain division scheme which divides the source domain into multiple sub-domains such that we can initiate a meta-learning framework for domain generalization. The sub-domain division is dynamically refined during the meta-learning. Next, in order to disentangle domain-invariant information from domain-specific information in image features, we design the domain-invariant and -specific crowd memory modules to re-encode image features. Two types of losses, i.e. feature reconstruction and orthogonal losses, are devised to enable this disentanglement. Extensive experiments on several standard crowd counting benchmarks i.e. SHA, SHB, QNRF, and NWPU, show the strong generalizability of our method.

==> Fig/visden2.tex <==
\begin{figure*}[t]
\begin{center}

\includegraphics[width=\linewidth]{Fig/visden2.png}
\end{center}

\caption{Qualitative examples of MAN~\cite{lin2022cvpr}, ours, and ground truth~(from left to right) on {SHA$\rightarrow$SHB / QNRF and SHB$\rightarrow$SHA / QNRF}.} 
% Here, target domain consists of train/test sets because we set a crowd counting dataset as target domain. 
%Domain Adaptation fine-tunes the trained model using target domain data
% ~(without using labels here) 
%and test the adapted model on the target domain test data. Domain generalization trains a model on the source domain and directly tests it on the target domain without target domain data and parameter updates. }
% 

%is introduced to measure the relative counts among local regions. Ground truth mask $A^g$ is used to optimize the attention module. Operations including upsampling and concatenation, as well as ground truth density maps $E^g$ are omitted for concise.
\label{fig:visden2}
\end{figure*}

==> Tab/abcluster.tex <==
\begin{table}[!t]
\centering

    % \resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c}

		\toprule
		Source  & \multicolumn{2}{c|}{SHA}  & \multicolumn{2}{c}{SHB}\\
		\midrule
		 Target &  SHB &  QNRF & SHA & QNRF\\
		 \midrule
		 K=2 & 18.3& 141.4 & 127.5& 194.7\\
		 K=3 & 14.6 & 128.7& \textbf{122.8} & \textbf{179.1} \\
		 K=4 &\textbf{12.5} & \textbf{120.2}& 132.4 & 193.2\\
		 K=5 & 16.5 & 121.3 & &\\
		 \midrule
		 E=1 & \textbf{12.5} &\textbf{120.2} & \textbf{122.8}&\textbf{179.1}\\
		 E=2 & & & &\\
		 E=5 & & & &\\
		 
		


		\bottomrule
	\end{tabular}
    % }
	\caption{Parameter Selection.}
	\label{tab:ablationcluster}	

\end{table}

==> Tab/comparison3.tex <==
\begin{table*}[!t]

\footnotesize
\centering

    % \resizebox{\linewidth}{!}{
	\begin{tabular}{c|cc|cc|cc|cc|cc|cc}

		\toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{CSRNet} & \multicolumn{2}{c|}{DMCount} & \multicolumn{2}{c|}{D2CNet} & \multicolumn{2}{c|}{SASNet} & \multicolumn{2}{c|}{MAN} & \multicolumn{2}{c}{\textbf{OURS}}\\
         & \multicolumn{2}{c|}{\scriptsize{\cite{li2018cvpr}}} & \multicolumn{2}{c|}{\scriptsize{\cite{wang2020nips}}} & \multicolumn{2}{c|}{\scriptsize{\cite{cheng2021tip}}} & \multicolumn{2}{c|}{\scriptsize{\cite{song2021aaai}}} & \multicolumn{2}{c|}{\scriptsize{\cite{lin2022cvpr}}} & \\
        \midrule
        \multicolumn{13}{c}{Generalizing to NWPU}\\
        \midrule
         \textit{Source} & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE\\
         \midrule
         SHA& 164.8 & 610.7 & 146.9 & \zp{563.8?} & 153.1 & \zp{548.9?} & 158.8 & 588.0 & 148.2 & 586.5 & \textbf{143.1} & {567.6}\\
         SHB & 179.1 & \zp{622.9?} & 191.6 & 747.4 & 206.1 & 770.2 & 195.7 & 716.8 & 193.6 & 802.5 & \textbf{175.0} & {688.6}\\
         SHA+SHB & 169.6 & 619.2 & 144.6 & 592.8 & -- & -- & 155.3 & 583.6 & 147.8 & 605.3 & \textbf{139.6} & \textbf{553.6}\\
         \midrule
         \multicolumn{13}{c}{Inverse Generalization from QNRF} \\
         \midrule
         \textit{Target} & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE\\
         \midrule
         SHA & 77.0 & 122.7 & 73.4 & 135.1 & 66.0 & 112.4 & 73.9 & 116.4 & 67.1 & 122.1 & \textbf{65.5} & \textbf{108.2}\\
         SHB & 12.0 & 21.7 & 14.3 & 27.5 & 16.1 & 27.5 & 13.0 & 22.1 & 12.5 & 22.2 & \textbf{11.1} & \textbf{20.0} \\


		\bottomrule
	\end{tabular}
    % }
	\caption{Comparison on generalization to NWPU~(The upper half). And inverse generalization from QNRF~(The lower half).}
	\label{tab:comparison2}	
	

\end{table*}

==> Tab/comparisonNWPU.tex <==
\begin{table*}[!t]
\begin{minipage}{0.55\textwidth}

\centering

    % \resizebox{\linewidth}{!}{
	\begin{tabular}{c|cc|cc|cc}

		\toprule
        Target: NWPU & \multicolumn{2}{c|}{SHA} & \multicolumn{2}{c}{SHB} & \multicolumn{2}{c}{SHA+SHB}\\
        \midrule
        Method & MAE & MSE & MAE & MSE & MAE & MSE \\
        \midrule
        CSRNet & 164.8 & 610.7 & 179.1 & 622.9\\
        DSSINet & 171.6 & 620.3 & 232.5 & 839.5\\
        D2CNet & 153.1 & 548.9 & 206.1 & 770.2\\
        % BL & 179.9 & 691.0 & 175.5 & 579.8\\
        SASNet & 158.8 & 588.0 & 195.7 & 716.8 & 155.3 & 583.6\\
        MAN & 148.2 & 586.5 & 193.6 & 802.5 & 147.8 & 605.3\\
        \midrule
        \textbf{OURS} & \textbf{143.1} & \textbf{567.6} & \textbf{175.0} & \textbf{688.6} & \textbf{139.6}& \textbf{553.6}\\


		\bottomrule
	\end{tabular}
    % }
	\caption{Comparison with state-of-the-art methods on NWPU.}
	\label{tab:comparisonNWPU}	
	
\end{minipage}
\hfill
\begin{minipage}{0.44\textwidth}
\centering

    % \resizebox{\linewidth}{!}{
	\begin{tabular}{c|cc|cc}

		\toprule
        Source: QNRF & \multicolumn{2}{c|}{SHA} & \multicolumn{2}{c}{SHB}\\
        \midrule
        Method & MAE & MSE & MAE & MSE \\
        \midrule
        D2CNet & 66.0& 112.4& 16.1 & 27.5\\
        DMCount & & & &\\
        SASNet & & & & \\
        MAN & 67.1& 122.1& 12.5& 22.2\\
        \midrule
        OURS & 73.0& 133.2& 11.1 & 20.0\\


		\bottomrule
	\end{tabular}
    % }
	\caption{An inverse generalization from QNRF to SHA and SHB.}
	\label{tab:inverse}	
\end{minipage}

\end{table*}

==> Tab/dataset.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{c|c|c|c|c}
    \toprule   
    \multicolumn{2}{c|}{Dataset} & \#Train & \#Test & [Min\_cnt, Max\_cnt]\\
    \midrule
    \multirow{2}{*}{SHTech} & part\_A & 300 & 182 & 33 $\sim$ 3139 \\\cmidrule{2-5}
    & part\_B & 400 & 312 & \\
    \midrule
    \multicolumn{2}{c|}{QNRF} &  & 334 & \\
    \midrule
    \multicolumn{2}{c|}{JHU} \\
    \midrule
    \multicolumn{2}{c|}{NWPU} \\
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:datasets}
\end{table}

==> Tab/inverse.tex <==
\begin{table}[!t]


\end{table}

==> sec2_relatedwork.tex <==
\section{Related Work}

\subsection{Crowd counting } Current mainstream approach for crowd counting is to learn a neural network to predict a density map, whose integration indicates the total crowd count in the image. Many works focus on improving model framework~\cite{jiang2020cvpr,liu2021iccv,lin2022cvpr}, learning target~\cite{wang2021iccv,song2021iccv,xiong2022eccv}, or introducing novel loss functions~\cite{ma2019iccv,wang2020nips,wan2021cvpr}. These methods bring large improvements to in-distribution test data, but contribute less to out-of-distribution performance. 
% \miaojing{rewrite this: In practice, training and test data xxxx, domain shift, xxx } 
{In real world application, there often exists a domain shift between training and test data, which would lead to possible failure of trained models.}
% Clearly, the practical value of deep crowd counting models for real-world applications are not promised with these fully-supervised approaches.

\noindent \textbf{Domain adaptive crowd counting.} To tackle the domain shift problem in crowd counting, many works rely on the domain adaptation (DA) technique~\cite{wang2019cvpr,sindagi2020eccv,he2021aaai,liu2022cvpr,gong2022cvpr}. DA adapts a model learned from a source domain to a target domain, where the target data is normally (partially) available, labeled or unlabeled, for model training or fine-tuning~\cite{he2021aaai,reddy2021tmm,wu2021mm}. For instance, ~\cite{reddy2020wacv,wang2021tnnls,hossain2019bmvc} have developed few-shot learning methods by assuming a few labeled data are available in the target domain for model finetuning. 
%which train the base model in the source domain with a large amount of labeled data and adapt the model to the target domain with only a few labeled data.
%\miaojing{rewrite this in more details}
% For example, AdaCrowd~\cite{reddy2021tmm} regards different camera scenes as different domains and learns to adapt to novel camera scenes. 
The crowd data in the source domain can sometimes be synthetic data~\cite{wang2019cvpr,sindagi2020eccv,zhang2021cvpr,liu2022cvpr,gong2022cvpr}, as they are much easier to obtain and label.
% ~\zp{The model learned on synthetic data will be transferred to real-world data by .} 
% \zp{~\cite{yan2021tcsvt} also tests their model on unseen dataset to evaluate the generalizability. Instead, we are the first to focus on solving domain generalization, and we are only accessing to a single domain. }\zp{few-shot->last}
% usually focuses on Unsupervised Domain Adaptation~(UDA), which adapts the trained model to target domains without annotations. UDA aims at eliminating domain shift by aligning source and target distributions in the feature space. A popular method for feature alignment relies on adversarial learning~\cite{}. Adversarial learning methods extract domain-invariant features by introducing a minmax rule between the feature extractor and a domain discriminator. 


\subsection{Domain generalization}\label{sec:II-dg}
% Domain generalization methods can be divided into three categories: data augmentation, domain-specific, domain-invariant. The first is to devise novel augmentation techniques. The second is to learn domain-specific ensembles. The last is to extract domain-invariant/-agnostic knowledge.
Domain generalization (DG) methods study the model generalizability on out-of-distribution data. The difference between DA and DG is that DA can access both source and target data while DG only the source data. 
%making the task more challenging. 
Many DG methods focus on increasing the diversity of the source (training) data~\cite{volpi2018nips,yang2021nips,zhou2021arxiv,wang2021iccv}. For instance,~\cite{volpi2018nips,yang2021nips} augment the training data with adversarially perturbed samples.
%~\cite{zhou2021arxiv} synthesizes novel target domains using feature-level data MixUp.
% ~\cite{wang2021iccv} minimize the mutual information upper bound approximation between synthesized samples and the source ones; and~\cite{zhou2021arxiv} synthesizes novel target domains using feature-level mixup. 
%\miaojing{It's very confusing below this session, I can not edit. Also prototypes/memories have to occur here in order to be discussed later}
%Some works ~\zp{learn domain-specific knowledge by specially designed domain specific components and make inference based on the correlation between the test data and domain-specific information~\cite{xu2014eccv,mancini2018icip,seo2020eccv}.}
% ~\cite{seo2020eccv} propose a domain-specific normalization layer for each domain.~\cite{xu2014eccv,mancini2018icip} choose to learn domain-specific classifiers and combine multiple domain-specific outputs during inference.
% ; for inference, multiple domain-specific outputs are combined by either simply averaging, measuring similarities between target domain and source domains, or using a deep architecture to predict weight vectors. 
Other methods focus on learning domain-invariant knowledge from the source domain. 
% ~\cite{li2018aaai} extends model-agnostic meta-learning~(MAML)~\cite{finn2017icml} to model-learning domain generalization~(MLDG). Many works follow up this meta optimization strategy to perform DG~\cite{}.
%Some methods resort to extract domain-invariant features.
For instance, ~\cite{lin2021iccv, zhang2022arxiv} achieve this by explicitly disentangling between domain-invariant and domain-specific representations in image features.  %{\cite{matsuura2020aaai,chen2022cvpr} study single-source domain generalization by dividing the source domain into multiple sub domains .}
Besides, memory/prototype networks are
often employed in DG to maintain categorical information across domains~\cite{chen2021iccv,kim2022cvpr,dai2021cvpr}. For instance,~\cite{chen2021iccv,kim2022cvpr} employ external memory to store domain-invariant class representations for image classification and semantic segmentation, respectively. % ~\cite{dai2021cvpr} learn prototypes to store individual information for person re-id.}

\noindent \textbf{Meta-learning domain generalization.} Meta-learning has also been popularly used to solve DG. 
%The seminal work, ~\cite{finn2017icml}, was originally proposed in few-shot learning learning. {It introduces an episodic training paradigm that divides the whole task (class) set into base and novel tasks to learn model adaption.}
The representative work, meta-learning domain generalization (MLDG) ~\cite{li2018aaai} which extends from model-agnostic meta-learning~(MAML) ~\cite{finn2017icml}, divides the source domain into meta-train and -test sets to simulate the domain shift between training and test. 
This episodic meta optimization strategy makes model parameters agnostic to domains. 
Many follow-up works employ this strategy to solve DG in different tasks, \eg semantic segmentation~\cite{kim2022cvpr}, face recognition~\cite{guo2020cvpr}, and person re-id~\cite{song2019cvpr,zhao2021cvpr,dai2021cvpr,ni2022cvpr}. 
% A popular way is to learn domain-agnostic parameters using gradient based meta-learning.
% Amounts of works follow up the meta optimization strategy in MLDG~\cite{li2018aaai}, which is the extension of model-agnostic meta-learning~(MAML)~\cite{finn2017icml} to DG.

\subsection{Domain-general crowd counting}\label{sec:dgcounting}
We propose the first work to solve DG in crowd counting. Our key components are both novel in crowd counting and also prominent in domain generalization. Below we distinguish our work from some relevant works.  
%\miaojing{introduce memory  and meta learning. 
%Memory/prototypes have been used in crowd counting but  we  Meta-learning has been used in crowd counting but we xxx}
%\zp{In this paper, we introduce meta learning and memory network to domain generalizable crowd counting. 

For meta learning, ~\cite{reddy2020wacv} has applied the MAML~\cite{finn2017icml} to few-shot crowd counting where few target data with labels are required. In contrast, our work utilizes MLDG~\cite{li2018aaai} for domain-general crowd counting where no target data/labels are required. Furthermore, we introduce new domain-invariant and -specific crowd memory modules and a dynamic sub-domain division scheme.
%During few-shot adaptation, several target data and their ground truth density maps are required, which are undesirable.
%On the other hand, we become the first to introduce the gradient-based meta learning method MLDG to simulate train-test domain shift for domain-generalizable crowd counting.

Memory networks have been employed in DG for solving other tasks~\cite{song2019cvpr,chen2021iccv,kim2022cvpr} (see Sec.~\ref{sec:II-dg}). Their memory vectors correspond to explicit categorical concepts (\eg object class, person id) and are initialized and iteratively updated by learned image features in the network. \cite{wu2021mm} have utilized this type of memory bank to build a domain-adaptive crowd counting model where each memory vector is defined as the mean head feature per image. Their model does not address the varying size and number of heads in crowd images, hence memory vectors can be subject to noise. 
%In fact, we argue that it is rather difficult to explicitly determine stored vectors in memory bank: density values are continuous, generating memory representation for each density value would be impossible; on the other hand, dividing the continuous density into discrete density levels may also suffer from quantization errors. To bypass this problem, 
Unlike them, we do not relate our memory vectors to explicit crowd concepts; instead, we initialize them as a set of random vectors. With properly devised loss functions, our memory vectors are implicitly learned as a set of density basis to re-encode image features into either domain-invariant or -specific features. Further differences to \cite{wu2021mm} include that we utilize memory vectors differently from them; they work for DA while we work for DG.     
%are initialized we introduce a novel domain-agnostic crowd memory that is automatically and implicitly updated with density-related domain-invariant feature vectors and enhanced through its orthogonality with domain-specific style information in domain-specific crowd memory.   
%in this procedure leads to inaccuracy and further needs refinement methods.   
%using network features at each training iteration.  
%explicitly store network features as domain-invariant class representations in memories or prototypes. However, in crowd counting it is difficult to  We think this approach inadequate because the size and number of heads vary both within and across images. Instead, we introduce a novel domain-agnostic crowd memory that is automatically and implicitly updated with density-related domain-invariant feature vectors and enhanced through its orthogonality with domain-specific style information in domain-specific crowd memory. 


Finally, in crowd counting, there are also some works studying multi-domain joint learning~\cite{yan2021tcsvt,chen2021variational}. Unlike us, they focus on improving the performance on multiple source domains and their model designs are also fundamentally different from ours. Notice ~\cite{chen2021variational} also conducts domain division: they train a variational attention module for Gaussian mixture clustering; samples from different datasets are re-grouped for follow-up training. Ours differs from it: we use K-Means clustering and dynamically refine clustering results by taking advantage of updated domain-specific information in image features.

% \miaojing{rewrite below} 
% we observe that both meta-learning and prototype/memory networks are widely used in tasks like classification, semantic segmentation, but rarely in crowd counting. The exceptions are~\cite{reddy2020wacv,wu2021mm}. \cite{reddy2020wacv} applied the established MAML to achieve few-shot crowd counting. However, few-shot learning requires several target data and their labels, which is undesirable. On the other hand, Based on the above observations, we become the first to introduce MLDG to crowd counting for DG. And more importantly, we introduce a novel meta memory module that is automatically updated with density-related feature vectors and enhanced through its orthogonality with domain-specific style information.
